Rational Sensibility: LLM Enhanced Empathetic Response Generation Guided by Self-presentation Theory

The development of Large Language Models (LLMs) provides human-centered Artificial General Intelligence (AGI) with a glimmer of hope. Empathy serves as a key emotional attribute of humanity, playing an irreplaceable role in human-centered AGI. Despite numerous researches aim to improve the cognitive empathy of models by incorporating external knowledge, there has been limited attention on the sensibility and rationality of the conversation itself, which are vital components of the empathy. However, the rationality information within the conversation is restricted, and previous methods of extending knowledge are subject to semantic conflict and single-role view. In this paper, we design an innovative encoder module inspired by self-presentation theory in sociology, which specifically processes sensibility and rationality sentences in dialogues. And we employ a LLM as a rational brain to decipher profound logical information preserved within the conversation, which assists our model in assessing the balance between sensibility and rationality to produce high-quality empathetic response. Experimental results demonstrate that our model outperforms other methods in both automatic and human evaluations.

==> table/ablation_case1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{p{7.835em}p{40.665em}}
    \toprule
    \multirow{3}[2]{*}{\textbf{Context}} & \multicolumn{1}{l}{\textit{Speaker:} hi, i feel so lonely sometimes because all my friends live in a different country} \\
    \multicolumn{1}{l}{} & \multicolumn{1}{l}{\textit{Listener:} oh, i am sure you are lonely. maybe you can join some kind of club that lets you meet new friends?} \\
    \multicolumn{1}{l}{} & \textit{Speaker:} i was thinking about it! i wanted to join a group for local moms \\
    \midrule
    \textbf{Emotion Cause} & i was thinking about it ! i wanted to join a group for local moms \\
    \textbf{LLama2} & Based on the dialogue content, the speaker is expressing a feeling of loneliness due to their friends living in a different country. The sentiment label is questioning, as the speaker is seeking suggestions for meeting new friends in their local area. The causal link between the dialogue content and the sentiment label is that the speaker's feeling of loneliness is driving their desire to seek out new social connections. \\
    \midrule
    \textbf{with conect} & that sounds like a good idea. i hope you enjoy it! \\
    \textbf{with self-pres} & that is awesome. i am sure you will be able to meet new people! \\
    \textbf{Ours}  & that is a good idea. maybe you could see if you could join some sort of club? \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:ablation_case1}%
\end{table}%


==> table/human_ab.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Results of Human A/B test.}
  
    \begin{tabular}{l|ccc}
    \toprule
    \textbf{Models} & \textbf{Win} & \textbf{Loss} & \textbf{Tie} \\
    \midrule
    Lamb vs EmpDG & 48.9\% & 15.3\% & 35.8\% \\
    Lamb vs CEM & 40.4\% & 18.7\% & 40.9\% \\
    Lamb vs SEEK & 41.2\% & 19.1\% & 39.7\% \\
    Lamb vs KEMP & 45.4\% & 18.8\% & 35.8\% \\
    Lamb vs DCKS & 37.1\% & 20.5\% & 42.4\% \\
    \bottomrule
    \end{tabular}%
    
  \label{tab:human_ab}%
\end{table}%


==> table/prompt.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \caption{The prompt used in CoNECT.}
    \begin{tabular}{m{1.1cm}p{15em}}
    \toprule
    Name  & \multicolumn{1}{c}{Content} \\
    \midrule
    Context & \textbf{speaker}: too often , it is a health scare that makes us  value health . It inspires me to try and do something to keep healthy every day .  \\
    Emotion & Hopeful \\
    Prompt & Suppose you are a psychiatrist with empathy. Given the following dialogue and the overall dialogue sentiment label, please briefly analyze the causal link between the dialogue content and the sentiment label.\newline{}\newline{}Dialogue content:\colorbox{yellow}{\{Context\}}\newline{}Dialogue sentiment label:\colorbox{yellow}{\{Emotion\}} \\
    \bottomrule
    \end{tabular}%
  \label{tab:prompt}%
\end{table}%

